Efficient chaining of seeds in ordered trees

We consider here the problem of chaining seeds in ordered trees. Seeds are mappings between two trees Q and T and a chain is a subset of non overlapping seeds that is consistent with respect to postfix order and ancestrality. This problem is a natural extension of a similar problem for sequences, and has applications in computational biology, such as mining a database of RNA secondary structures. For the chaining problem with a set of m constant size seeds, we describe an algorithm with complexity O(m2 log(m)) in time and O(m2) in space.

==> chaining2D.tex <==

\section{Seeds borders intervals}\label{sec:algo}

Each border node of a seeds corresponds to a location where the seed will possibly 
linked with descendants to form a chain. For example, if $b$ is a leaf of a 
seed $P$, then the chain made of $P$ and a chain included in $\widehat{Q_b}$
and $\widehat{T_b^P}$ is a valid chain. If $b$ is not a leaf, then 
 some of its descendants are in $P$ (not necessarily direct children). Between 
theses descendants, there are couples of forests where it is possible to find 
chains that can be linked with $P$. 

The following definitions aims at formally specifying these couples of forests for 
a border node:

\begin{definition}\em Given a seed $P$ on a tree $T$ and a forest $V=T[a,b]$ 
free of $P$'s nodes ($P\cap V=\emptyset$).

$V$ is {\em left maximal} if $T_{a-1}$ contains at least one $P$'s node. The highest
node of $P$ contained in $T_{a-1}$ is called the  {\em left limit} 
of $V$.

In the same way, $V$ is {\em right maximal} if $b+1$ is a descendant of at least one 
$P$'s node. The lowest node of $P$ ancestor of $b+1$ (can be $b+1$) is called 
the {\em right limit} of $V$.
\end{definition}

\begin{figure}
\begin{center}\includegraphics[width=0.9\linewidth]{figures/border}
\caption{Exemplification of chainable areas. On the left, the case of a border node $b$ that is a leaf of $P$. On 
the right, the maximal forests $V_0$, $V_1$, $V_2$ for $b$ and the left and right limits of $V_1$.}
\label{fig:below}
\end{center}
\end{figure}

\begin{definition}\em Let $b$ be a border node of the seed $P$ between two 
trees $Q$ and $T$. We define by
$F(b)=\{((a_i,b_i),(c_i,d_i))\}$ the set of all couples of forests 
in $\widehat{Q_b}\times\widehat{T_{b^P}}$ encoded by their indices on 
$[l(b);b[^2 \times [l(b^P);b^P[^2$  such that for all $((a_i,b_i),(c_i,d_i))$
in $F$:
\begin{itemize}
\item $a_i<b_i$ and $c_i<d_i$ (forests are non empty)
\item There is no $x$ in $P$ such that $a_i \le x \le b_i$ or $c_i \le x^P \le d_i$
(forests are free of $P$'s nodes).
\item $a_i=l(b)$ and $c_i=l(b^P)$, or, there exists a $y$ in $P$ such that $y \in Q_{a_i-1}$ and $y^P \in T_{c_i-1}$
(forests are left maximal and their left limits form a mapping in $P$).
\item There exists a $z$ in $P$ such that $b_i+1 \in Q_{z}$ and $d_i+1 \in T_{z^P}$
(forests are maximal on the right side and their right limits form a mapping in $P$).
\end{itemize}
$F(b)$ will be referred as the {\em chainable areas} of $b$.
\end{definition}


It follows from this definition that if $b \in L(P)$ then 
$F(b)={((l(b),b-1),(l(b^P),b^P-1))}$. Thus, if $b$ is a leaf,
$F(b)$ represents the couple of forests $\widehat{Q_b}$
and $\widehat{T_{b^P}}$ as stated early.

A more complicated example is if we suppose $b$ to have 
$\ell$ children $c_0 \dots c_{\ell-1}$ and only $c_i$ is in $P$. 
In that case, $F_b=\{((l(b),(l(c_i)-1)),(l(b^P)),(l(c_{i}^P)-1)),
((c_i+1,b-1),(c_{i}^P+1,b^P-1))\}$. The first couple corresponds
to the forests below $(b,b^P)$ on the left of $(c_i,c_{i}^P)$ and 
the second couple corresponds to the forest under $(b,b^P)$ on 
the right of $(c_i,c_{i}^P)$ (theses forests could possibly be empty 
in which case they do not appear in $F(b)$).

On Figure~\ref{fig:below}, $F(b)=\{((5,12),(2,8))\}$. It is left maximal 
as node $4$ of $Q$ is in $P$ and is the root of $Q_{4=5-1}$
and its image $1$ in $T$ is the root of $T_{1=2-1}$. It is also right maximal
as $13$ is in $P$ and $Q_{13}$ contains $12+1$ and
$T_{9=13^P}$ contains $8+1$.



\section{Combinatorial properties of chains and seeds}
\label{sec:2D-preliminaires}

We first describe combinatorial properties of chains between trees,
that naturally leads to a recursive scheme to compute a maximum chain
(Section~\ref{sec:preliminaires}). 

We consider in the following a tree $T$ and a node $i$ of $T$. The
first leaf visited during a postfix traversal of $T_i$ is denoted by
$l(i)$ and called the {\em leftmost leaf} of the node $i$. The ordered
forest induced by the proper descendants of $i$ is denoted by
$\widehat{T_i} = T[l(i),i-1]$.

Let $P$ be a seed, $b$ be a node of $T$ that belongs to
$B(T_P)$. $Ch_P(T,b)$ is the list of children of $b$ that also belong
to $T_P$, ordered by their postfix number. The list may be empty
($Ch_P(T,b)=\emptyset$) if $b$ is a leaf of $T_P$, which is the case
of all border nodes if $P$ is compact. If
$B(T_P)=\{b_0,\ldots,b_{m-1}\}$, we denote by $deg_T(P)$ the sum
$\sum_{j=0,\ldots,m-1}|Ch_P(T,b_j)|+1$; by definition of chains, if
$P$ is a seed between trees $Q$ and $T$, then $deg_T(P)=deg_Q(P)$, and
we then denote both by $deg(P)$. Property~\ref{prpy:degree} below
follows immediately from the fact that any border node of an internal
tree $T_P$ which is not a leaf of $T_P$ is ancestor of a leaf of
$T_P$.

%Commentaire Pascal : Je mettrai cette propriété après la propriété 2,
%comme un corollaire de cette propriété, il me semble que la preuve
%découle justement directement de la propriété 2. Sinon il faudrait
%mettre au moins une idée de la preuve.
%Commentaire Cedric : fait ci-dessus.
\begin{property} \label{prpy:degree} Given an internal tree $T_P$ of a tree $T$,
$deg_T(P) \le 2\times |B(T_P)| +1 $.
\end{property}

Next, let us describe how the subtrees of $T$ rooted in the nodes of
the border of $P$ can be decomposed into forests.
% Commentaire Pascal :  je pense que la phrase  suivante n'est pas
% utile et prèt à confusion 
%  Later, these forests
% will be central to introduce the decomposition of a maximum chain
% into smaller chains located into these forests.
We denote by $F_P(T,b)$
the list of (possibly empty) forests defined as follows:
\begin{itemize}
\item  if $Ch_P(T,b)=\emptyset$: then $F_P(T,b)=T[l(i),i-1]$
($F_P(T,b)$ contains a single forest, which is empty if $T[i]$ is a leaf
of $T$), 
\item if $Ch_P(T,b)=\{i_0,\ldots,i_{k-1}\}$ with $k >0$: then
  $F_P(T,b)=\{T[l(b),l(i_0)-1],T[i_0+1,l(i_1)-1],\ldots,T[i_{k-2}+1,l(i_{k-1})-1],T[i_{k-1}+1,b-1]\}$
  (See Figure~\ref{fig:below} for an illustration).
\end{itemize}
We denote by $F^k_P(T,b)$ the $k^{th}$ forest of $F_P(T,b)$, for
$k=0,\ldots,|Ch_P(T,b)|$. 

\begin{figure}
\begin{center}\includegraphics[width=0.7\linewidth]{figures/example2}
\caption{$Ch_P(Q,b)=(3,4,13)$. $F_p(Q,b)=(Q[0,1], Q[4,3], Q[5,12],
  Q[14,13])$.
  $Ch_P(T,b^P)=(0,1,10)$. $F_P(T,b^P)=(T[0,-1],T[1,0],T[2,8],T[11,10])$.}
\label{fig:below}
\end{center}
 \vspace*{-5mm}
\end{figure}

The next property describes the structure of any chain between two
trees $Q$ and $T$ given a set of $m$ seeds
$S=\{P^0,\ldots,P^{m-1}\}$. In the following, for a node $u$ in $Q$ of
a given seed $P^j$ in $S$, we denote by ${u^j}$ the unique node in $T$
such that the pair $(u,u^j)$ belongs to the mapping that defines
$P^j$.

\begin{property}
  \label{prpy:structure_chain}
  Let $P^j$ be the last seed of a chain $C$. $C$ can be decomposed
  into $deg(P^j)+2$ (possibly empty) distinct chains: $P^j$, a chain
  $C'$ between $Q[0,l(r_j)-1]$ and $T[0,l(r_j^j)-1]$, and, for every
  pair $(b,b^j) \in P^j$ and every $k=0,\ldots,|Ch_{P^j}(Q,b)|$, a
  chain between $F^k_{P^j}(Q,b)$ and $F^k_{P^j}(T,b^j)$.
\end{property}

The proof of this property is a direct consequence of the constraints
that define a mapping, and implies that each distinct chain in the
decomposition of $C$ is a chain between a subforest of $Q$ and a
subforest of $T$. The following property is then straightforward.

%Commentaire Pascal: Il me semble que cette propriété est difficile à
%lire pour quelqu'un qui n'est pas dans le sujet. Je me demande s'il
%ne faudrait pas introduire une notation algébrique pour décrire la
%décomposition d'une chaine en plusieurs chaines.
\begin{property}
  \label{prpy:structure_opt_chain}
  Let $P^j$ be the last seed of a maximal chain $C$. Each non-empty
  chain of the decomposition of $C$ as described in
  Property~\ref{prpy:structure_chain} is a maximal chain between the
  corresponding forests.
\end{property}

%PASCAL: j'ai changé les références à "maximal chain" ou "optimal
%chain" en "maximum chain" qui me parait plus juste et consistant avec
%ce qu'on a introduit.
Property~\ref{prpy:structure_opt_chain} naturally leads to a recursive
scheme to compute an optimal chain between two trees $Q$ and $T$:
The pairs of vertices of $Q$ and $P$ that belong to the mappings defining
the seeds of $S$ are scanned according to the postfix order of the
nodes in $Q$, and for the current pair $(b,b^j)$ (belonging to the
seed $P^j$ then), if $b$ is the root of $P^j$ then we look for a
maximal chain between $Q[0,l(r_j)-1]$ and $T[0,l(r_j^j)-1]$, and if
$b$ is in the border of $P^j_Q$, we look for maximum chains between
the forests $F^i_{P^j}(Q,b)$ and $F^i_{P^j}(T,b^j)$, for all pertinent
values of $i$.

%PASCAL : Il faut reformuler le paragraphe suivant CEDRIC : Autant le
%supprimer car il prend de l'espace et engendre plus de confusion que
%de clart\'e. 
%PASCAL : parfait :)
%% Note that the only difference between the general scheme we described
%% and chaining algorithms in sequences occurs when we process a seed
%% root, as it requires to compute a maximal chain located to the left of
%% $b$ in $Q$ and $b^j$ in $T$ is required, which does not happen in
%% sequences that are equivalent to unary trees. There lies the
%% algorithmic challenge that requires to design data structures and
%% control structures that handles this ``left'' constraint efficiently.

Let $P$ be a seed between two trees $Q$ and $T$, $b$ a node of $Q$
that belongs to $B(Q_P)$ and $c$ the node of $T$ such that $(b,c)\in
P$ (so $c\in B(T_P)$). By definition of a seed,
$|Ch_P(b)|=|Ch_P(c)|=k$ for some non-negative integer $k$. We
denote by $F_P(b)$ the set $\{f_0,\ldots,f_k\}$ of $k+1$ quadruples
such that $f_i=(i_1,i_2,i_3,i_4)$ if and only if $F_P(Q,b)=Q[i_1,i_2]$
and $F_P(T,c)=T[i_3,i_4]$. Hence, $F_P(b)$ encodes the postfix numbers
of the first and last nodes of the forests in $Q$ and $T$ where
maximum subchains are seeked.
% PASCAL: Je ne comprends pas bien le paragraphe précédent, notamment
% pourquoi c n'apparait pas dans la notation  $F_P(b)$  alors qu'il me
% semble que la liste de noeuds dépends de b et de c.

\begin{lemma}\label{lem:forests}
  Given a set $S=\{P^0,\ldots,P^{m-1}\}$ of closed seeds between two
  ordered trees $Q$ and $T$, all the lists $F_{P^j}(b)$ for all seeds
  $P^j$ and all border nodes $b$ of $P^j$ can be computed in
  $O(||S||\log(||S||))$ time and $O(||S||)$ space.
\end{lemma}

To prove the above lemma, we only need to notice that once the pairs
$(b,b^j)$ of the mappings defining the seeds of $S$ are ordered
increasingly according the the postfix number of the nodes of $Q$,
then the lists $F_{P^j}(b)$ can be computed during a single reading of
the mapping pairs, because we consider closed seeds. The space
complexity follows from Property~\ref{prpy:degree}.

%% ------------------------------------------------------------------
\section{An algorithm solving the Maximal Chaining Problem}
\label{sec:2D}

We first describe a simple but non-optimal implementation of this
scheme (Section~\ref{sec:algo-imp1}), based on the properties
described in the previous section, followed by a more efficient one
(Section~\ref{sec:algo-imp2}).

From now, we assume that we are given two ordered trees $Q$ and $T$, a
set $S=\{P^0,\ldots,P^{m-1}\}$ of closed seeds, with $P^0=(r_Q,r_T)$
(it contains a single pair composed of the roots of $Q$ and $T$), and
that the score $v(j)$ of a seed $P^j$ can be accessed in constant
time.  We also assume that the seeds $P^j$ are given as a list $I$ of pairs
$(i,r,j)$ where $i$ is the postfix number of a node of $Q$ that is
either root or border of the seed $P^j$ and $r$ indicates if $i$ is
either border, or root or both for $P^j$; as a preprocessing, we sort
$I$ in increasing order of the first field (postfix number in $Q$). We
also consider that the lists $F_{P^j}(b)$ for all border nodes of the
seeds are available and that, for a node $i$ in $Q$ belonging to a
seed $P^j$, the corresponding node in $T$, $i^j$ (or more precisely its
postfix number in $T$) can be accessed in constant time. Finally, we
assume that for every node $i$ in $Q$ and $T$, its leftmost leaf
$l(i)$ can be accessed in constant time. In both algorithm, we visit
the elements in $I$, and a seed is said to be {\em visited} after its
root has been visited.

\subsection{A simple non optimal implementation}
\label{sec:algo-imp1}

We first present an implementation, whose main interest is to be very
simple as it requires no special data structure.  

The key point is to handle the request to find maximal subchains in
$O(1)$ time.  To achieve the desired complexity, we maintain two data
structures: an array $V$ of $m$ integers and an array $M$, indexed by
quadruples $(a,b,c,d)$ of integers. We also make use of a function
\texttt{Update} that takes an entry $M[a,b,c,d]$ and a value $w$ and replace
the value of this entry by $w$ if and only if $w > M[a,b,c,d]$.  The
correctness of the algorithm relies on the following invariants:
\begin{itemize}
\item[M1.] $M[a,b,c,d]$ is the value of the maximum chain included into
$(Q[a,b],T[c,d])$ composed only of visited seeds.
\item[V1.] $V[j]$ is the score of the best chain formed of $P^j$ and
  of visited seeds contained in both $Q_{r_j}$ in $Q$ and in
  $T_{{r^j_j}}$ in $T$.
\end{itemize}

%Anne-Laure : ancienne version compacte
%\begin{algorithm}
%\caption{$MCP_1(Q,T,S,v)$: compute a  maximal chaining from $S$.}
%\label{alg:second_version}
%\begin{lstlisting}
%|$I$: list of seeds borders and root nodes in $Q$, sorted in increasing postfix number
%|$V$: array of size $k$, initially $V[j]=v[j]$ for every seed $j$ in $S$
%for $i$ in $I$ do
%  if $i$ is a border of $P^j$ then $V[j]= V[j]+M[l[i],i-1,l[{i^j}],{i^j}-1]$
%  else # $i$ is the root of $P^j$, $i=r_j$
%    foreach $v$ ancestor of $i$, border of a seed $h$ s.t. ${v^h}$ is ancestor of ${r^j_j}$ do
%      $w = V[j]+M[l[v],l[r_j]-1,l[{v^h}],l[{r^j_j}]-1]$
%      Update $M[l[v],v,l[{v^h}],{v^h}]$ with $w$
%      foreach $r_g$ s.t. $l[r_g] \in ]r_j,v[$ and $l[{r^g_g}] \in ]{r^j_j},{v^h}[$ do
%        Update $M[l[v],l[r_g]-1,l[{v^h}],l[{r^g_g}]-1]$ with $w$
%\end{lstlisting}
%\end{algorithm}

\begin{algorithm}
\caption{$MCP_1$: compute the score of a  maximal chain.}
\label{alg:second_version}
\begin{lstlisting}
for $j$ from $0$ to $m-1$ do $V[j]=v(j)$
for $i$ in $I$ do
  if $i$ is a border of $P^j$ then 
     foreach $(a,b,c,d) \in F_{P^j}(i)$ do $V[j]= V[j]+M[a,b,c,d]$
  else # $i$ is the root of $P^j$, $i=r_j$
    foreach $v$ ancestor of $i$, border of a seed $P^h$ s.t. ${v^h}$ is ancestor of ${r^j_j}$ 
      and $\exists (a,b,c,d) \in F_{P^h}(v)$ s.t. $r_j \in [a,b]$ and $r^j_j \in [c,d]$ do
      $w = V[j]+M[a,l(r_j)-1,c,l({r^j_j})-1]$
      Update $M[a,b,c,d]$ with $w$
      foreach $r_g$ s.t. $l(r_g) \in ]r_j,v[$ and $l({r^g_g}) \in ]{r^j_j},{v^h}[$ do
        Update $M[a,l(r_g)-1,c,l({r^g_g})-1]$ with $w$
return $\max_{j} V[j]$
\end{lstlisting}
\end{algorithm}

To prove the correctness of the algorithm, we need to show that
property V1 is satisfied, as it implies that $\max_{j} V[j]$ contains
the score of the maximal chain. It follows from both
Property~\ref{prpy:structure_chain} and the fact that $V$ is updated
only at line 4, that V1 is satisfied if M1 is satisfied for all
entries $M[a,b,c,d]$ such that $(a,b,c,d)\in F_{P^j}(i)$. Hence we
only need to show that M1 is satisfied for quadruples $(a,b,c,d)$ that
belong to $F_{P^j}(i)$ for some node $i$ of $Q$ border of a seed
$P^j$. Moreover, an entry of $M$ needs only to be modified when a new
seed that is contained in the forests it defines in $Q$ and $T$ is
visited, which is done at lines 6-11.

The space complexity is in $O(m||S||)$, due to the space required to
encode $M$, as each entry is indexed either by a quadruple
$(l[v],r_g,l[v^j],r_g^g)$ for some border node $v$ of a seed $P^j$ and
root $r_g$ of some seed $P^g$, or by a quadruple
$(l[i],i-1,l[i^j],i^j-1)$ where $i$ is a border node. The time
complexity is in $O(m^3+||S||\log(||S||))$. The $m^3$ term is due to the
double loop in lines 7-11 that can have up to $O(m^2)$ iterations (due
to the fact that seeds are compact) and is performed once for each
root of the $m$ seeds. The $||S||\log(||S||)$ is due to sorting $I$.

%% CEDRIC: STOP ICI, DIMANCHE 21 MARS.

\subsection{A more efficient implementation}
\label{sec:algo-imp2}

We describe now an alternative implementation, whose goal is to
achieve the complexity stated in Theorem~\ref{thm:main}. Note that
here again, we first describe only how to compute the score of a
maximal chain.Computing an optimal chaining can be done using standard
backtracking techniques and will be described in the full version of
this paper.

The idea is to access less entries from $M$ (while maintaining
property M1 on the required entries though) and complement $M$ with a
data structure $R$ that can be queried in $O(\log(m))$ instead of
$O(1)$, but whose maintenance does not require a loop with $O(m^2)$
iterations.  More precisely $R$ is defined as follows:
\begin{itemize}
\item $R$ is indexed by all pairs of leaves $(l_Q,l_T)$ such that
  $l_Q$ is a leaf of $Q$, $l_T$ a leaf of $T$ and there is a border
  node $v$ of a seed $P^j$ such that $l[v]=l_Q$ and $l[v^j]=l_T$;
\item Each $R[l_Q,l_T]$ contains a set of pairs $(y,s)$ such that
  $P^y$ is the last seed of some valid  chain $C$ and $s$ is the
  score of $C$.
\end{itemize}
Moreover, $R$ satisfies the following properties:
\begin{itemize}
\item[R1.] For each entry $(y,s)$ of $R[l_Q,l_T]$ representing a chain
  $C$, the first seed $P^z$ of $C$ satisfies $r_z\geq l_Q$ and
  $r_z^z\geq l_T$.
\item[R2.] If $R[l_Q,l_T]=((y_0,s_0),\ldots,(y_p,s_p))$, then for
  every $i\in\{1,\ldots,p-1\}$, $r_{y_i}^{y_i}<r_{y_{i+1}}^{y_{i+1}}$ and
  $s_i<s_{i+1}$.
\item[R3.] After visiting node $i$ of $Q$, for each $(y,s) \in
  R[l_Q,l_T]$ (for any $l_Q,l_T$), there is no chain in
  $(Q[l_Q,i],T[l_T,r_y^y])$ with a score larger than $s$.
\end{itemize}

% Anne-Laure version non compacte
%\begin{algorithm}
%\caption{$MCP_2(Q,T,S,v)$: compute a  maximal chaining from $S$.}
%\label{alg:third_version}
%%\begin{minipage}[]{0.5\textwidth}
%\begin{lstlisting}[firstnumber=0]
%|$I$: list of seeds borders and root, and leftmost leaves of seeds roots, sorted in increasing postfix number in $Q$
%|$V$: array of size $k$, initially $V[i]=v[i]$ for every seed $j$ in $S$
%|$X$: list of pairs $(l[v],l[v^j])$ for all border $v$ of a seed $P^j$, sorted in increasing postfix number in $Q$
%foreach $i$ in $I$ do
%  if $i=l[r_j]$ then
%    foreach $(l[v],l[{v^h}]) \in X$ s.t. $l[v],l[{v^h}] < l[r_j],l[{r^j_j}]$ do
%      Update $M[l[v],l[r_j]-1,l[{v^h}],l[{r^j_j}]-1]$ with  the last $(y,s)$ of $R[l[v],l[{v^h}]]$ s.t. $r_y^y < l[{r^j_j}]$
%  else if $i$ is a border of $P^j$ then # add a loop if seeds are not compact
%    Add to $V[j]$ the last $(y,s)$ of $R[l[i],l[{i^j}]]$ s.t. $r_y^y < {i^j}$
%  else # $i$ is the root of $P^j$, $i=r_j$
%    foreach $(l[v],l[{v^h}]) \in X$ s.t. $l[v],l[{v^h}] < l[r_j],l[{r^j_j}]$ do
%      $w = V[j]+M[l[v],l[r_j]-1,l[{v^h}],l[{r^j_j}]-1]$
%      Insert entry $(j,w)$ into $R[l[v],l[{v^h}]]$
%\end{lstlisting}
%%\end{minipage}
%\end{algorithm}


\begin{algorithm}
\caption{$MCP_2(Q,T,S,v)$: compute a  maximal chaining from $S$.}
\label{alg:third_version}
%\begin{minipage}[]{0.5\textwidth}
\begin{lstlisting}[]
|$I$: list of seeds borders and root, and leftmost leaves of seeds roots, sorted in increasing postfix number in $Q$
|$V$: array of size $k$, initially $V[i]=v[i]$ for every seed $j$ in $S$
|$X$: list of pairs $(l[v],l[v^j])$ for all border $v$ of a seed $P^j$, sorted in increasing postfix number in $Q$
foreach $i$ in $I$ do
  if $i=l[r_j]$ then
    foreach $(a,c) \in X$ s.t. $a,c < l[r_j],l[{r^j_j}]$ do
      Update $M[a,l[r_j]-1,c,l[{r^j_j}]-1]$ with  the last $(y,s)$ of $R[a,c]$ s.t. $r_y^y < l[{r^j_j}]$
  else if $i$ is a border of $P^j$ then 
    foreach $(a,b,c,d) \in F_{P^j}(i)$ do
      Add to $V[j]$ the last $(y,s)$ of $R[a,c]$ s.t. $r_y^y < d$
  else # $i$ is the root of $P^j$, $i=r_j$
    foreach $(a,b,c,d) \in X$ s.t. $a,c < l[r_j],l[{r^j_j}]$ do
      $w = V[j]+M[a,l[r_j]-1,c,l[{r^j_j}]-1]$
      Insert entry $(j,w)$ into $R[a,c]$
\end{lstlisting}
%\end{minipage}
\end{algorithm}




A key point here is the algorithm to insert an entry $(j,w)$ into
$R[l[v],l[{v^h}]]$ in line 12, while ensuring that property R2 is
satisfied. It is achieved by replacing line 12 by the following:
\begin{lstlisting}[firstnumber=12]
find the last entry $(y,s)$ s.t. $r_y^y < r_j^j$
if $s < w$ then 
  insert $(j,w)$ just after $(y,s)$ in $R[l[v],l[{v^h}]]$
  remove from $R[l[v],l[{v^h}]]$ all entries $(z,t)$ s.t. $r_j^j < r_z^z$ and $t < w$
\end{lstlisting}

Note that the score of a maximal  chain in $(Q,T)$ is available as
the best entry in $R[0,0]$.
  
\paragraph{Correctness of the algorithm.}
We first assume that properties R1, R2 and R3 are satisfied at any
time, and M1 is satisfied for a given entry when this entry is used
(lines 6 and 11). The correctness of the algorithm is a direct
consequence of the two following remarks.
\begin{enumerate}
\item Steps 7-8 of Algorithm~\ref{alg:third_version} implement step 4
  of Algorithm~\ref{alg:second_version}, and then step 4 of
  Algorithm~\ref{alg:overview}.
\begin{enumerate}
\item Clearly, entries of $R[l[i],l[{i^j}]]$ s.t. $r_y^y < {i^j}$ are
  valid chains belonging to $(\widehat{Q_i},\widehat{T_{i^j}})$.
\item The entries of $R[l[i],l[{i^j}]]$ are sorted by increasing score
  (property R2), and so, by property R3, the last entry s.t. $r_y^y <
  {i^j}$ is the best chain in $(\widehat{Q_i},\widehat{T_{i^j}})$.
\end{enumerate}
\item As property M1 is satisfied, steps 11-12 of
  Algorithm~\ref{alg:third_version} with $h=0$ correspond to steps 7
  and 8 with $h=0$ in Algorithm~\ref{alg:second_version}, and then to
  step 5 of Algorithm~\ref{alg:overview}. Updating $M$ is then
  replaced by updating $R$.
\end{enumerate}

We then need to prove that properties M1, R1, R2 and R3 are
satisfied. We first address the validity of properties R1 to R3.
\begin{itemize}
\item Property R1 is obviously satisfied following the query on $M$ in
  line 11 that defines the only inserted chains into $R$ in line 12.
\item Property R2 follows immediately from the insertion procedure
  used to insert new entries into $R$.
\item Finally, we prove that property R3 is satisfied. Let $(y,s)$ be
  an entry of $R[l_Q,l_T]$ representing a chain $C_1$. Assume that
  there is a better chain $C_2$ in $(Q[l_Q,i],T[l_T,r_y^y])$.  

  If the last seed $P^z$ of $C_2$ satisfies $r_z < r_y$, we can assume
  without loss of generality that $C_2$ is the best such chain. This
  implies that $C_2$ was present into $R[l_Q,l_T]$ before $(y,s)$, as
  it was inserted when $i=r_z$. As $r_z^z < r_y^y$, then the insertion
  procedure into $R$ prevents $(y,s)$ to be inserted. 

  Otherwise, the last seed $P^z$ of $C_2$ satisfies $r_z > r_y$, and
  the entry $(y,s)$ will be removed during step 4 of the insertion of
  $(z,t)$ into $R[l_Q,l_T]$.
\end{itemize}


Finally, we address the validity of property M1. From property R3, the
last $(y,s)$ of $R[l[v],l[{v^h}]]$ s.t. $r_y^y < l[{r^j_j}]$
represents the best chain in
$(Q[l[v],l[r_j]-1],T[l[v^h],l[r_j^j]-1])$. Moreover, all chains that
have still to be considered (i.e. that contain at least one inactive
seed) have a last seed with a root that is larger than $l[r_j]-1$ in
$Q$ which implies that they would not impact on the considered M entry
and then that the entry of $M$ considered at line 6 is correct when it
is used. For line 11, as the entry of $M$ is used after it was updated
at line 6, property M1 is satisfied for this entry.


\paragraph{Complexity of the algorithm.}
For the space complexity, it is given by the space required for
structures $M$ and $R$. Every entry in $M$ is defined by a border node
and a root node in $Q$, and similarly in $T$, which gives a $O(m||S||)$
space. For $R$, each $R[l_Q,l_T]$ is defined by a border node and
contains $O(m)$ entries, which gives an $O(m||S||)$ space.

Following the technique used for computing maximal chains in
sequence~\cite{Gusfield-algorithms,Joseph-determining,Ohlebusch-chaining},
the structures $R[l_Q,l_T]$ can be implemented using classical data
structures such as AVL supporting query requests, insertions and
deletions in a list of $n$ elements in $O(\log(n))$ worst-case time.

If we do not consider line 15 (removing entries from some
$R[l_Q,l_T]$), it is easy to see that the time complexity is in
$O(m||S||\log(m)+||S||\log(||S||))$. First, the term $||S||\log(||S||)$ comes
from sorting $X$. Next there are $k$ seeds roots (hence each
$R[l_Q,l_T]$ contains $O(m)$ entries) and the list $X$ contain
$O(||S||)$ entries, which implies that lines 4-6 of
Algorithm~\ref{alg:third_version} have a $O(m||S||\log(m))$ time
complexity.  Lines 7-8 have clearly a $O(||S||\log(m))$ time
complexity. Finally, as for lines 4-6, lines 10-14 have a
$O(m||S||\log(m))$ time complexity. We then only need to measure the
impact of line 15, that removes entries from the lists in $R$. It
follows from property R2 that all removed entries are consecutive in
$R[l_Q,l_T]$. Hence the amortized complexity of this step is linear in
the total number of removed entries. As there are at most $O(m||S||)$
entries in $R$, this gives an amortized $O(m||S||)$ time complexity for
step 15, which completes the complexity analysis.

If we consider that $Q$ and $T$ are sequences, or, as described in
Section~\ref{sec:preliminaries}, unary trees, then each of the two
trees has a single leaf and $||S||=m$. This implies that $R$ contains a
single element, that is a list of $O(m)$ entries. Similarly, as
entries of $M$ that are required are indexed by quadruples of leaves,
there are at most $m$ such entries, and the total space complexity is
then in $O(m)$. The fact that each tree has only one leaf also implies
that loops at lines 5-6 and 10-15 have each a single iteration, which
reduces the time complexity by a factor $O(m)$ and give a $O(||S||\log
(m))=O(m\log(m))$ time complexity.



